Zero-Shot Transfer of Neural ODEs

Autonomous systems often encounter environments and scenarios beyond the scope of their training data, which underscores a critical challenge: the need to generalize and adapt to unseen scenarios in real time. This challenge necessitates new mathematical and algorithmic tools that enable adaptation and zero-shot transfer. To this end, we leverage the theory of function encoders, which enables zero-shot transfer by combining the flexibility of neural networks with the mathematical principles of Hilbert spaces. Using this theory, we first present a method for learning a space of dynamics spanned by a set of neural ODE basis functions. After training, the proposed approach can rapidly identify dynamics in the learned space using an efficient inner product calculation. Critically, this calculation requires no gradient calculations or retraining during the online phase. This method enables zero-shot transfer for autonomous systems at runtime and opens the door for a new class of adaptable control algorithms. We demonstrate state-of-the-art system modeling accuracy for two MuJoCo robot environments and show that the learned models can be used for more efficient MPC control of a quadrotor.

==> plots/vanderpol_plot.tex <==
% Define grid dimensions
\def\numCols{4}
\def\numRows{2}
\def\plotWidth{4cm}
\def\plotHeight{4cm}
% \def\horizontalGap{0.5cm}
% \def\verticalGap{0.5cm}
\newcommand{\muvalue}{-1}

% Loop through rows and columns to create plots
\foreach \row in {1,...,\numRows} {
    \foreach \col in {1,...,\numCols} {
        \pgfmathsetmacro{\index}{\col - 1 + (\row-1) * \numCols)}
        \pgfmathsetmacro{\xtrue}{int(4*\index)}
        \pgfmathsetmacro{\ytrue}{int(4*\index + 1)}
        \pgfmathsetmacro{\xlearned}{int(4*\index + 2)}
        \pgfmathsetmacro{\ylearned}{int(4*\index + 3)}
        \pgfmathsetmacro{\result}{0.41428571428 * \index + 0.1}
        \renewcommand{\muvalue}{
        \num[round-mode=places, round-precision=2,exponent-mode=fixed]{\result}
        }
        % \pgfmathsetmacro{\muvalue}{0}
        \subfloat[$\mu=\muvalue$]{
        \begin{tikzpicture}

        \begin{axis}[
            width=\plotWidth,
            height=\plotHeight,
            xmin=-2.3,
            xmax=2.3,
            ymin=-5.2,
            ymax=5.2,
            xticklabels={}, % Disable x-axis tick labels
            yticklabels={}, % Disable y-axis tick labels
            ]
            
            % plot true dynamics
            \addplot[black] table [col sep=comma, x index=\xtrue, y index=\ytrue] {data/vanderpol/vanderpol_comparison_neuralODE.csv};
            
            % plot neural ode
            \addplot[red] table [col sep=comma, x index=\xlearned, y index=\ylearned] {data/vanderpol/vanderpol_comparison_neuralODE.csv};

            % plot FE neural ODE
            \addplot[blue] table [col sep=comma, x index=\xlearned, y index=\ylearned] {data/vanderpol/vanderpol_comparison_FE_neuralODE.csv};        
            
            
            \end{axis}
        \end{tikzpicture}
        }
    }
}

